An Empirical Study on Package-Level Deprecation in Python Ecosystem

Open-source software (OSS) plays a crucial role in modern software development. Utilizing OSS code can greatly accelerate software development, reduce redundancy, and enhance reliability. Python, a widely adopted programming language, is renowned for its extensive and diverse third-party package ecosystem. However, a significant number of OSS packages within the Python ecosystem are in poor maintenance, leading to potential risks in functionality and security. Consequently, it is essential to establish a deprecation mechanism to assist package developers and users in managing packages effectively. To facilitate the establishment of the package-level deprecation mechanism, this paper presents a mixed-method empirical study, including data analysis and surveys. We investigate the current practices of announcing, receiving, and handling package-level deprecation in the Python ecosystem. We also assess the benefits of having deprecation announcements for inactively maintained packages. Furthermore, we investigate the challenges faced by package developers and users and their expectations for future deprecation practices. Our findings reveal that 75.4% of inactive package developers have no intention of releasing deprecation declarations for various reasons, while 89.5% of users express a desire to be notified about the deprecation, highlighting a gap between developers and users; in many cases, no alternative solutions are available when deprecation occurs, emphasizing the need to explore practical approaches that enable seamless package handover and require less maintenance effort. Our work aims to enhance the understanding of existing package-level deprecation patterns within the Python OSS realm and facilitate the development of deprecation practices for the Python community in the future.

==> 023Preliminary.tex <==
\section{Preliminary}
% Traditionally, to discourage consumers of OSS from adopting the deprecated functionality, developers of OSS use code-level deprecation mechanisms to send a warning \zq{add a reference about code-level deprecation mechanism}.
% In this paper, consumers of OSS refer to users who adopt OSS in their projects. 
% And some software ecosystems have package-level and release-level deprecation mechanisms to discourage consumers from adopting the deprecated package or a specific version, in case the project's developers give up maintaining or specific releases contain bugs \cite{cogo2021deprecation}.\slhe{wondering why don't we have a background section to put all these definitions there? package-level depre is too detailed here?} 
% % \slhe{explanations are needed here, people do not understand what different levels mean...}
% For instance, the deprecation mechanism in npm for JavaScript enables developers who want to deprecate their package to announce a deprecation message containing the rationale and the alternative for the package.
% In this paper, we specifically define deprecated packages as those packages with explicit deprecation announcements.

In this context, consumers of open-source software (OSS) are individuals who integrate OSS into their projects. 
In general, OSS developers employ code-level deprecation mechanisms to warn against adopting deprecated functionality, while some software ecosystems implement package-level and release-level deprecation mechanisms to discourage the adoption of deprecated packages or specific versions. These mechanisms are intended to discourage adoption when packages are no longer maintained, or certain releases contain bugs. For example, the npm deprecation mechanism for JavaScript allows developers to announce a deprecation message that specifies the rationale and alternative options for the package. In this study, we define deprecated packages as those that have explicit deprecation announcements.


Inactive packages, also referred to as dormant~\cite{valiev2018ecosystem}, abandoned~\cite{avelino2019abandonment}, halted ~\cite{pashchenko2018vulnerable}, unmaintained ~\cite{coelho2017modern} packages, receive poor maintenance in recent periods. 

Moreover, simply imitating the deprecation mechanism in other ecosystems rather than designing a specific one for the Python ecosystem would be confusing even though there are existing package and release level deprecation mechanisms in other ecosystems (e.g., npm for javascript, Cargo for Rust, etc.). It is because deprecation mechanisms in different ecosystems offer functionalities with different constraints. For example, the deprecation mechanism in .NET forces users to provide rationales if they perform a deprecation, while the deprecation mechanisms in javascript, Rust, and PHP do not set the constraint.
Given different designs of deprecation mechanisms, what is the most suitable pattern for the Python ecosystem remains unclear.
% In this context, consumers of open-source software (OSS) are individuals who integrate OSS into their projects. In general, OSS developers employ code-level deprecation mechanisms to warn against adopting deprecated functionality, while some software ecosystems implement package-level and release-level deprecation mechanisms to discourage adoption of deprecated packages or specific versions. These mechanisms are intended to discourage adoption when projects are no longer maintained, or certain releases contain bugs. For example, the npm deprecation mechanism for JavaScript allows developers to announce a deprecation message that specifies the rationale and alternative options for the package. 

==> 03ResearchQuestions.tex <==
\section{Research Questions}
The main goal of this paper is to investigate the status quo of package-level deprecation in the Python ecosystem and to provide guidelines for the future development of a deprecation mechanism at the package level for the Python ecosystem.
To reach this end, we conducted an mix-method empirical study leveraging several sources of data, including PyPI for the release history of all packages, GitHub for additional package characteristics, and Snyk for information on vulnerabilities.

In the expansive Python ecosystem, with its numerous of third-party packages, there remains ambiguity regarding the exact number of those that are inactive.
% \zq{not related to the research questions}
Furthermore, there remains uncertainty regarding the possibility to find a deprecation declaration for inactive packages, a factor that may deter consumers from adopting these packages.
Despite the presence of deprecation declarations within the packages, the lack of a unified package-level deprecation mechanism has led to an absence of consensus about the content that should be included in these declarations, and the appropriate locations for their publication.
As a result, consumers are left unsure about where they can access the deprecation declarations, and what information they can expect to obtain from them.
% With no unified package-level deprecation mechanism currently in place, even though there are deprecation declarations in the packages, there is no consensus on what content should be included in the deprecation declarations and where these deprecation declarations should be published.
% Therefore, consumers are uncertain about that where they can access the deprecation declarations, and what content they can obtain from the deprecation declarations.
% For example, the deprecation mechanism in .NET forces users to provide rationales if they perform a deprecation, while the deprecation mechanisms in Javascript, Rust, and PHP do not set the constraint.
% For example, it is necessary to provide rationales before developers deprecate a package in .NET ecosystem, while there is no such constraint in javascript, Rust, and PHP.
% % there is no existing one for the Python ecosystem. 
% There are various types of package-level deprecation mechanisms, but the best practice has been unclear.
% It is essential to investigate what kind of deprecation mechanism suits the Python ecosystem best.
To gain a better understanding of the current overview of package-level deprecation in the Python ecosystem, we ask:

\begin{itemize}[leftmargin=*]
    \item \textbf{RQ1. How package-level deprecation of Python package is made?}
\end{itemize}
% \textbf{RQ1. How package-level deprecation of Python package is made?}

%  Adopting inactive projects may introduce vulnerabilities \zq{example}. 
% How explicit announcements stop the propagation is still unclear.
While prior work has highlighted the disadvantages of adopting inactive packages \cite{decan2018impact}, 
it is observed that people still adopt inactive packages, potentially incorporating outdated or even vulnerable code into their projects \cite{synopsys2023open,pashchenko2018vulnerable, alfadel2023empirical}. 
This may be due to the ambiguity in recognizing inactive packages without clear deprecation declarations.
% This adoption may be influenced by the ambiguity consumers face when deciding whether to use an inactive package without an explicit deprecation declaration, leading them to believe that there is still value in using the package. 
Although the Python community has discussed deprecation mechanisms for years \cite{naveen2021deprecate,Gedam2022adding}, no tangible solutions have been realized.
% In this context, we see potential in package-level deprecation declarations to mitigate the issue.
% In this context, we explore the potential of package-level deprecation declarations to address the issue.
% People ..., the value of explicit announcements has been unclear.
% We hypothesize that explicit deprecation declarations could deter new consumers from adopting the package and encourage existing consumers to migrate to alternative packages, which would subsequently manifest as reduced adoption of the deprecated packages by other packages in the ecosystem. We refer to this phenomenon as the decrease of downstream dependency after the deprecation declarations are published.
% Additionally, we anticipate that explicit deprecation declarations would help prevent new consumers from encountering bugs or problems, sending issues that might not receive a response from official members
In this context, we explore the potential of package-level deprecation declarations to address the issue. 
We hypothesize that explicit declarations could deter new users and encourage migration to alternatives, reducing the overall adoption of deprecated packages.
This could decrease downstream dependency (i.e., adoption from other dependents in PyPI) and help prevent new users from encountering unresolved issues or bugs \cite{toda2019characterizing, valiev2018ecosystem}.
To verify the hypothesis, we assess the deprecated packages based on the gain of downstream dependency and the number of unresolved issues after the deprecation.
If these metrics decrease, it would indicate that such a declaration is effective in reducing ambiguity and clarifying the risks associated with using the package. Therefore, we pose the following question: \textbf{RQ2. How do deprecation declarations impact the gain of downstream dependencies and unresolved issues?}
% \begin{itemize}[leftmargin=*]
%     \item \textbf{RQ2. How do deprecation declarations impact the gain of downstream dependencies and unresolved issues?}
% \end{itemize}
% \noindent\textbf{RQ2. How do deprecation announcements impact the gain of downstream dependencies and unresolved issues?}

% As we have seen the ratio of deprecated with an explicit announcement may be low. 
% To investigate the factors that indicate higher probabilities of making an explicit deprecation announcement.
% We further study the differences in attributes and characteristics between deprecated packages and other categories.
% We ask:

% Beyond the prevalence of deprecation among inactive projects, there may be more characteristics that affect the effectiveness of deprecation announcements.


% While explicit declarations in packages exist, the absence of a unified package-level deprecation paradigm presents numerous challenges for consumers.
% One such challenge is the difficulty consumers face in locating declarations due to variations in publishing locations \cite{millerwe}, leading to low efficiency in the declaration process.
% Additionally, the lack of consensus within the community on the content that should be included in the deprecation declaration may result in ineffective dissuasion from adopting deprecated packages.
% Establishing a package-level deprecation mechanism could help unify the deprecation paradigm.
% However, the question remains: What type of deprecation mechanism, or alternatively, what type of deprecation declaration, could effectively alleviate the situation? 
% One natural idea is referring to existing package-level deprecation mechanisms in other ecosystems, such as npm for javascript or Cargo for Rust.
% Nevertheless, these deprecation mechanisms offer different functionalities, and some even impose constraints on the deprecation process.
% For instance, the .Net ecosystem requires developers to provide rationales before deprecating a package, while no such constraint exists in Javascript, Rust, and PHP ecosystems.
% Merely imitating one of these mechanisms might not be the optimal solution to address the challenges specific to the Python ecosystem.
% Hence, it is essential to investigate what type of deprecation mechanism suits the Python ecosystem best.
% To provide guidelines for developing a package-level deprecation mechanism for the Python ecosystem, we aim to investigate the factors that contribute to an effective deprecation declaration. This investigation includes examining the location of deprecation declarations (e.g., published in README or in issues) and the content of these declarations (e.g., replacement and rationale).
% To facilitate developing an effective deprecation mechanism, understanding what made a deprecation announcement effective is essential. 

While packages do contain explicit declarations, the absence of a unified deprecation paradigm poses challenges for consumers.
These challenges include difficulties in locating declarations due to diverse publishing locations \cite{miller2023we}, resulting in inefficient deprecation message delivery. Moreover, the lack of consensus on content may fail to deter the adoption of deprecated packages.
To provide valuable insights that can inform the development of future deprecation announcement systems for Python, we aim to investigate the characteristics of effective deprecation declarations, including the publishing location and included content.
(e.g., published in README or in issues) and the content of these declarations (e.g., replacement and rationale)
% \zq{Establishing a unifying mechanism could help, but the question of its form remains. 
% One idea is referring to existing mechanisms like npm for JavaScript or Cargo for Rust.
% However, their diverse functionalities and constraints, such as the .Net requirement for rationales, may not suit Python.
% Simply imitating one of them might not address Python-specific needs.
% Therefore, our goal is to investigate what suits Python best, including examining the location of deprecation declarations (e.g., published in README or in issues) and the content of these declarations (e.g., replacement and rationale), to guide a package-level deprecation mechanism's development.}
We ask:
% \noindent\textbf{RQ3. What characteristics of the projects indicate the deprecation?}

\begin{itemize}[leftmargin=*]
    \item \textbf{RQ3. What are the characteristics of an effective deprecation declaration?}
\end{itemize}
% \noindent\textbf{RQ3. What are the characteristics of an effective deprecation announcement?}

The following section gives an overview of our study design to answer the three research questions.

==> 04StudyOverview.tex <==
\section{Study Overview}
We have conducted an empirical study, meticulously designed to analyze data from multiple sources, including PyPI, GitHub and Snyk.

The study is divided into of two main parts. The first part focuses on exploring the patterns of package-level deprecation (i.e., \textit{RQ1}), while the second part delves into examining the impact of deprecation declarations and their characteristics (i.e., \textit{RQ2, RQ3}).
For a more detailed discussion on the methods used to address each research question, please refer to \hyperref[sec:Methods]{section 5}.

To address \textit{RQ1}, we established a pool of inactive packages using a mixed-method filtering approach. 
Within this pool, we manually verified packages that are marked as deprecated and include a deprecation declaration in their corresponding GitHub repositories. 
% both proactive method and passive methods\zq{is sending an e-mail and waiting for a response kind of passive method?}.

Regarding \textit{RQ2}, we aim to investigate the impact of deprecation declaration from two aspects, the prevention of unresolved issues \cite{valiev2018ecosystem}, and the prevention of an increase in downstream dependencies.
To achieve this, we employed linear mixed-effect (llm) models.
To address \textit{RQ3}, we extended these models by incorporating relevant deprecation declaration characteristics as predictors.

==> 05Methods_old.tex <==
\section{Methods}
\label{sec:Methods}
In this section, we detail all our operations.


\subsection{Data Collection}
To address our three research questions, we aggregated data from a diverse array of sources, including PyPI, GitHub, and Snyk \cite{snyk2023vulnerability}.
%including metadata of the python packages, vulnerabilities in PyPI and GitHub statistics. 


Specifically, we initially retrieved metadata for all 415,151 available packages as of January 09, 2023, using the official PyPI API. We focused on obtaining the release history and the corresponding GitHub link, if available.
The release history is essential in the metadata as it provides insights into the package's life activity, potentially indicating the next release date \cite{pashchenko2018vulnerable}.
% For the release history, we download the distributions to extract the dependency of the release. 
For each release, we downloaded one of the distributions to extract the dependency information.
Furthermore, we accessed the corresponding GitHub repository via the link in the metadata to collect additional data, such as stars, README, issues, contributors, and commit histories utilizing the GitHub REST API\footnote{https://docs.github.com/en/rest?apiVersion=2022-11-28}. 
% Besides, we also collect the corresponding GitHub link in the metadata to collect more data from GitHub. 
% After we get access to the GitHub repository of the projects, we collect the data, including stars, README, issues, contributors and commit histories using GitHub REST API\footnote{https://docs.github.com/en/rest?apiVersion=2022-11-28}. 
Finally, we obtained 2,996 vulnerabilities with 35,304 affected versions from Snyk \cite{snyk2023vulnerability}, a leading software composition analysis (SCA) companies.
Out of these vulnerabilities, 2,857 (95.3\%) were resolved in subsequent versions.
% It is note worth noting that Snyk records vulnerabilities more than CVE. \zq{is it true}

\subsection{Identifying Deprecation}
\label{sec:identifing}
We first identified inactive packages from the entire set of 415,151 packages on PyPI, following the approaches used in prior works \cite{pashchenko2018vulnerable, khondhu2013all, coelho2017modern, kula2018developers, valiev2018ecosystem, ait2022empirical}. 
Next, we then conducted keyword searches in the corresponding GitHub repositories to identify potential signs of deprecation.
Specifically, we search for a list of keywords (e.g., deprecated, unmaintained, not maintained 
anymore, etc.) in both README and the issues created after the last commit.
Finally, we manually inspect the repository to determine whether any packages containing these keywords have an explicit deprecation declaration.

Since most of the methods used in prior works are rule-based, their effectiveness can be a threat to validity. In other words, these methods may incorrectly identify packages that are actually under-maintained as inactive.
To mitigate this threat, we categorize these methods into two groups and select one method from each category to identify inactive packages, thereby increasing the likelihood of accuracy.
% from each category we choose one method to filter out the inactive packages for a higher possibility.
% \zq{an example about fp here?} \zq{why are the two definitions most representative}.

One category of methods reads the latest commit history and takes a certain commit amount or longest duration without commit as metrics to identify inactive packages. 
For example, Khondhu et al., Coelho et al. and Kula et al. consider packages as inactive packages if there has been no commit in the last year \cite{khondhu2013all, coelho2017modern, kula2018developers}. 
Valiev et al. consider the projects as inactive projects if the projects had less than one commit per month on average in the last 12 months prior to the last commit \cite{valiev2018ecosystem}.
While Ait et al. consider projects as inactive projects if there is no activity in the last 6 months \cite{ait2022empirical}.
Among these metrics, we finally adopted the rule, which identifies packages without commit on the corresponding GitHub repository in the last year, as the representative of this category.

The other rule we considered is based on the concept of "halted package", which was introduced by Pashchenko et al. \cite{pashchenko2018vulnerable}. 
According to this concept, a package is considered halted if it exceeds the expected time to release a new version, based on its release history. 
% \zq{more explanations from the original paper?}
Specifically, we have Equation~\ref{eq:next_release_date} which adopts an Exponential Smoothing model to calculate the next expected release date \cite{brown1959statistical}. 
In this model, greater weight is assigned to the more recent release intervals compared to the older intervals. 
% while calculating the Next release interval. 
% Packages that exceed the date to release a new version will be identified as halted packages.
% \begin{equation}
% \label{eq:next_release_date}
% \begin{aligned}
% Next\ release\ interval &= \alpha \sum^{n-1}_{i=0}\{(1-\alpha)^i\ast Release\ time_{n-i-1}\} \\ 
% Expected\ release\ date &= Next\ release\ interval \\
% &+ Last\ release\ date
% \end{aligned}
% \end{equation}
\begin{equation}
\label{eq:next_release_date}
\small % change the font size command here
\begin{aligned}
Next\ release\ interval &= \alpha \sum^{n-1}_{i=0}\{(1-\alpha)^i\ast Release\ time_{n-i-1}\} \\ 
Expected\ release\ date &= Next\ release\ interval \\
&+ Last\ release\ date
\end{aligned}
\end{equation}
Where $\alpha$ denotes a smoothing parameter that ranges in $(0,1)$, here we take the value as 0.6 as Pashchenko et al. do \cite{pashchenko2018vulnerable}, $n$ denotes that there are $n$ intervals in the release history (i.e., $n+1$ releases), and $Release\ time_i$ denotes the time needed to release a new version after the \textit{i}-th version.
% Pashchenko et al. adopted an Exponential Smoothing model \cite{brown1959statistical} to assign a bigger weight for the recent release intervals compared to the intervals of the older releases while calculating the Next release interval.

By adopting the concept of a halted package as the rule, we identified 255,296 halted packages. 
% However, there are some cases that it is hard to determine it as halted packages as the intervals of the release history are too short.
% For example, aaa/bbb.
Additionally, we applied the rules that consider projects without any commits in the last year, resulting in the identification of 122,402 packages that meet this criterion.
% Similarly, there are also cases that we can hardly determine it as inactive package, since some of the projects have a slow pace to update their project.
% We also provide an example here.
To address the potential threat to validity, we combined both rules together and identified 89,193 inactive packages, forming our dataset, These inactive packages constitute 21.5\% of the entire PyPI as of January 09, 2023.
% As a result, there are 89,xxx inactive packages we labeled to study in this paper.
% We sample xxx packages using a sample calculator.

% The key idea is that we want to measure the probability for a consumer to obtain the deprecation announcement via passive way (the announcement is shown in README or issues) or active way (i.e., asking through email).\zq{whether asking via email is different from the definition of deprecation, i.e., explicit announcement}
To explore the corresponding GitHub repositories of inactive packages, we conducted keyword searches for a list of frequently used sentences in README and official replies in issues created after the last commit \cite{coelho2018identifying}. 
If any of the identified sentences were found in the repository, we manually inspected it to determine the presence of a package-level deprecation declaration.

\subsection{Dependency Network}
In our analysis, we specifically consider packages that are explicitly declared as dependencies in other PyPI packages.  
This means dependencies that are not part of the PyPI ecosystem, such as system dependencies and GitHub projects that do not originate from PyPI are excluded. 
% \zq{maybe a reference here?}
Additionally, optional extras \cite{collins2015pep0508, coghlan2012pep0426} are outside the scope of our research as they are not required for package installation.
In the context of a package in PyPI, we use the term "upstream packages" or "upstream dependencies" to refer to packages that are used by the current package. Conversely, "downstream packages" or "downstream dependencies" are packages that depend on the current package. 
% \zq{Is there a necessity here? Since we might use other words in the following section.}

To ensure comprehensive and current dependency information, we extracted this data from distribution files of each version, following the approach of prior work \cite{valiev2018ecosystem}.
Specifically, PyPI supports two types of distributions for a package: built distribution and source distribution.
Initially, we focused on the built distribution as it contains machine-readable metadata for dependencies.
In cases where built distributions are not available, we conducted a mimic installation with the source distribution in the sandbox environment.
During this process, we logged the dependencies required for the installation. 
In total, we obtained dependency information from 4,034,194 releases.

% \subsection{Compiling a Control Group}

\subsection{Propagation of Vulnerabilities}
Normally, when a Python package specifies its dependencies in the requirements, it may specify a range of versions of the dependencies that suit its need \cite{collins2015pep0508}.
% which means many versions of the dependencies are possible to be installed in different environments and different version constraints. 
Although 2,857 (95.3\%) of the vulnerabilities we collected were fixed in later versions, downstream dependencies can still be affected if they specify older, vulnerable versions of the package \cite{kula2018developers}.
In this paper, we determine whether a package contains vulnerability by traversing all its direct and transitive dependencies of the latest version of the package. 
If the package itself or its direct or transitive dependencies contain vulnerabilities, then we will consider it a vulnerable package.
Eventually, we detected 52,250 vulnerable packages in our inactive packages dataset, indicating the prevalence of vulnerabilities in the Python ecosystem.

\def\VariableName{3cm}
\def\DescLength{13cm}
\begin{table*}[h]
% \setlength{\tabcolsep}{50pt}
  \centering
  \caption{The definitions of the variables in our models}
  \label{tab:definitions}
  \begin{tabular}{ll}
    \toprule
    % Non-English or Math&Frequency&Comments\\
    % \midrule
    \multicolumn{2}{l}{\textbf{\textit{Outcome Variables}}} \\
    \parbox{\VariableName}{\vspace{.5\baselineskip}Gain of downstream dependencies\vspace{.5\baselineskip}} & 
     \parbox{\DescLength}{\vspace{.5\baselineskip}We define the gain of downstream dependencies in PyPI as follows: if only the latest version of a downstream package depends on the current package, we consider it an increase in downstream dependencies of the current package. Conversely, if there are versions other than the latest that depend on the current package, we consider it a decrease in downstream dependencies of the current package. The gain of downstream dependencies is then defined as the difference between the increase and decrease in downstream dependencies. \vspace{.5\baselineskip}} \\
     \parbox{\VariableName}{\vspace{.5\baselineskip}Gain of unresolved issues \vspace{.5\baselineskip}}  & 
     \parbox{\DescLength}{\vspace{.5\baselineskip}This variable refers to the number of GitHub issues that are in an open state and have not received any reply from any official member of the repository. Specifically, we consider issues that were created after the last commit to the repository. Since every consumer is also a tester of open-source software, it is common for them to report bugs and wait for help~\cite{breu2010information}. However, without a deprecation declaration to discourage consumers and potential users from adopting the package, it is possible that many reported bugs will not receive a reply in the GitHub issues.\vspace{.5\baselineskip}} \\ 
     \multicolumn{2}{l}{\textbf{\textit{Repository Characteristics}}}\\
      \parbox{\VariableName}{\vspace{.5\baselineskip}Project age \vspace{.5\baselineskip}}  & 
     \parbox{\DescLength}{\vspace{.5\baselineskip}Number of days since the first commit to the last commit.\vspace{.5\baselineskip}} \\
      \parbox{\VariableName}{\vspace{.5\baselineskip}Project stars \vspace{.5\baselineskip}}  & 
     \parbox{\DescLength}{\vspace{.5\baselineskip}Number of stars of the corresponding GitHub project.\vspace{.5\baselineskip}} \\
      \parbox{\VariableName}{\vspace{.5\baselineskip}Number of contributors \vspace{.5\baselineskip}}  & 
      \parbox{\DescLength}{\vspace{.5\baselineskip}
      %The VIF test revealed collinearity with the Number of original tweets and it was thus removed in the final model.%
      The number of contributors of the corresponding GitHub repository.
      \vspace{.5\baselineskip}}\\
      \parbox{\VariableName}{\vspace{.5\baselineskip}Number of releases \vspace{.5\baselineskip}}  & 
       \parbox{\DescLength}{\vspace{.5\baselineskip}Number of releases that were uploaded to PyPI.\vspace{.5\baselineskip}} \\
      \parbox{\VariableName}{\vspace{.5\baselineskip}Duration since last commit \vspace{.5\baselineskip}}  & 
       \parbox{\DescLength}{\vspace{.5\baselineskip}Number of days from the last commit to now (as of 2023.3.27).\vspace{.5\baselineskip}} \\
     \multicolumn{2}{l}{\textbf{\textit{Deprecation Declaration Characteristics}}}\\
      \parbox{\VariableName}{\vspace{.5\baselineskip}Published in README \vspace{.5\baselineskip}}  & 
       \parbox{\DescLength}{\vspace{.5\baselineskip}The deprecation declaration was made public in the README file of the corresponding GitHub repository. This declaration is visible to all visitors of the repository, even those who may not carefully inspect every detail.\vspace{.5\baselineskip}} \\
      \parbox{\VariableName}{\vspace{.5\baselineskip}Published in Issues \vspace{.5\baselineskip}}  & 
       \parbox{\DescLength}{\vspace{.5\baselineskip}The deprecation declaration was posted in a GitHub issue, typically in response to an inquiry about the project's maintenance status. Consumers need to exercise more caution to discover such declarations in GitHub issues.\vspace{.5\baselineskip}} \\
      \parbox{\VariableName}{\vspace{.5\baselineskip}Has rationale\vspace{.5\baselineskip}}  & 
     \parbox{\DescLength}{\vspace{.5\baselineskip}We consider whether the authors have provided a clear and understandable reason for launching the deprecation declaration. This characteristic is important because if the reason for deprecation is not significant (e.g., it does not involve security vulnerabilities that cannot be fixed), consumers may not see the need to perform a migration, which could involve potential refactoring costs.\vspace{.5\baselineskip}} \\
      \parbox{\VariableName}{\vspace{.5\baselineskip}Has alternative\vspace{.5\baselineskip}}  & 
     \parbox{\DescLength}{\vspace{.5\baselineskip}This characteristic refers to whether the authors of the deprecated repository have provided an alternative for it. We take this into consideration because consumers may be more willing to perform a migration if a viable alternative is offered \cite{brito2016developers}. \vspace{.5\baselineskip}} \\
  \bottomrule

\end{tabular}
\end{table*}

\subsection{Estimating Effect of Deprecation}
We aim to examine the effects of making an explicit deprecation declaration and identify the characteristics that contribute to its effectiveness.
% For \textbf{RQ2}
For each inactive package, we collected variables that capture the corresponding GitHub characteristics, and the variables related to the deprecation declarations, if available. 
We also record the measurements of the two dependent variables, namely the gain of GitHub unresolved issues on GitHub and the gain of downstream dependencies. 
For a comprehensive list of variables with their definitions, refer to table~\ref{tab:definitions}. 

% \noindent\textbf{Data Preparation}.
% Before we fit the models, we choose the subset of the inactive dataset to minimize the bias.
% First, we take all 8xx packages that are labeled as deprecated packages into consideration.
% For each deprecated package, we traverse the dependency network and find all its brother packages (i.e., have at least one common dependency) in the inactive dataset. \zq{why brothers}
% Instead of taking all its brothers into the subset, we only take the top 5 packages that have the closest number of stars in the corresponding GitHub repository.

\noindent\textbf{Model Specification.} To address \textit{RQ2} and \textit{RQ3}, we utilize Linear Mixed Effect Regression (lmer) models. 
% which is xxx \zq{usage}. 
% We chose glmer to estimate the effect of deprecations as well as their characteristics in terms of whether it can stop adoption from downstream dependencies since the output is binomial. \zq{find more explanation}
% We choose lmer to estimate the effect in terms of unanswered issues, for we can not reduce a binary variables from the amount of issues.
% We use \textit{glmer} from the \textit{lme4} \zq{need reference} package and the \textit{lmer} function from the \textit{lmerTest} package in R language \cite{kuznetsova2017lmerTest}.
We employed the \textit{lmer} function from the \textit{lmerTest} package in the R language \cite{kuznetsova2017lmerTest}.
The lmer model is represented by Equation~\ref{eq:deprecation}, where $Y$ represents the outcome variables, i.e., gain of downstream dependencies and the gain of unresolved issues.
$d$ is a boolean variable indicating the presence of a deprecation declaration,
and $r$ represents the repository characteristics.
The coefficients of the corresponding variables are denoted as $\beta_i$,
and the "owner-cohort" random effect is represented by $\delta$. 
When estimating the effect of having a deprecation declaration, we use Equation~\ref{eq:deprecation} to fit the lmer model, resulting in Model I and Model III.
To extend the analysis to include repository characteristics, we use Equation~\ref{eq:characteristics} to build Model II and Model IV.

\begin{equation}
\label{eq:deprecation}
\begin{aligned}
Y = \beta_0d  + \beta_1r+ \delta  
\end{aligned}
\end{equation}

\begin{equation}
\label{eq:characteristics}
\begin{aligned}
Y = \beta_0d * X+ \beta_1r + \delta 
\end{aligned}
\end{equation}

To answer \textit{RQ3}, we extend the model to incorporate $X$, which are the characteristics of deprecation declaration.

\noindent\textbf{Model Estimation.}
\label{sec:estimation}
Before building the models, we carefully select a subset of the entire inactive dataset to minimize bias.
Initially, we consider all 844 packages that are labeled as deprecated packages.
For each deprecated package, we traverse the dependency network and identify all its brother packages (i.e., have at least one common dependency) in the inactive dataset.
Instead of including all its brothers in the subset, we only select the top 5 packages that have the closest number of stars in the corresponding GitHub repository.
% For models that predict whether the propagation of downstream dependencies is stopped, we further exclude the packages that have had no downstream dependency ever since their first release.
Additionally, We take standard precautions when building the models as follows.
We use log-transforming variables to mitigate heteroscedasticity with skewed distributions \cite{gelman2006data}
except for the gain of downstream dependencies since it has negative values.
To check for multicollinearity, we use the \textit{Variance Influence Factor} (VIF) from the \textit{car} R packages~\cite{fox2019companion}. 
% We also report a marginal R-squared ($R^2_m$) and conditional R-squared ($R^2_c$) to indicate the goodness of fit. \zq{using what?}
% Our results (i.e., Table~\ref{tab:results}) are created by SjPlot package\zq{or by summary}.
% The Model I and Model II shows the the dependent variables as Predictors of the model, the Odds-Ratio that shows a effect on decreasing downstream dependencies when the value <1 and a effect on increasing downstream dependencies when the value >1) and the significance level. 
% The probability definition of odds-ratio is as the Equation~\ref{eq:odd_ratios}. 
% Let's take an example, if the value of odds ratio is 0.8 when the deprecation takes True as value (i.e., having a deprecation announcement), it means that the probability of increasing downstream is 20\% lower.

% \begin{equation}
% \label{eq:odd_ratios}
% \begin{aligned}
% prob=\frac{odds\_ratio}{1+odds\_ratio}
% \end{aligned}
% \end{equation}

==> 06Result.tex <==
\section{Results}
% \begin{figure*}[ht]
% 		\centering
% 		\includegraphics[width=0.90\linewidth]{Figures/RQ_1_characteristics.pdf}
% 		\caption{issues or README. \zq{need to be refined}}
% 		\label{fig:basic_characteristics}
% \end{figure*}

\begin{table*}
  \centering
  \caption{Overview of Our dataset}
  \label{tab:Overview}
  \begin{tabular}{llllcccccc}
    \toprule
    \multicolumn{2}{l}{Group} &\multicolumn{2}{l}{Variables} & min & 25\% & 50\% & 75\% & max & average\\
    \midrule
    \multicolumn{2}{l}{} &\multicolumn{2}{l}{Project stars} & 0.00 & 0.00 & 2.00 & 9.00 & 55928.00 & 37.01\\
    \multicolumn{2}{l}{} &\multicolumn{2}{l}{Project age} & 0.00 & 25.19 & 250.04 & 808.88 & 18974.86 & 567.41\\
    \multicolumn{2}{l}{} &\multicolumn{2}{l}{Number of contributors} & 1.00 & 1.00 & 2.00 & 3.00 & 2129.00 & 3.77\\
    \multicolumn{2}{l}{Entire Dataset (89,193)} &\multicolumn{2}{l}{Number of releases} & 2.00 & 3.00 & 5.00 & 9.00 & 1005.00 & 7.93\\
    \multicolumn{2}{l}{} &\multicolumn{2}{l}{Duration since last commit} & 372.46 & 696.39 & 1084.38 & 1770.89 & 4742.64 & 1324.39\\
    \multicolumn{2}{l}{} &\multicolumn{2}{l}{Delta of downstream dependencies} & -115.00 & 0.00 & 0.00 & 0.00 & 295.00 & -0.02\\
    \multicolumn{2}{l}{} &\multicolumn{2}{l}{Number of unresolved issues} & 0.00 & 0.00 & 0.00 & 0.00 & 1111.00 & 0.51\\
    % \cmidrule(lr){3-4}\cmidrule(lr){5-6}
    \midrule
    \multicolumn{2}{l}{} &\multicolumn{2}{l}{Project stars} & 0.00 & 2.00 & 12.00 & 59.00 & 21413.00 & 167.17\\
    \multicolumn{2}{l}{} &\multicolumn{2}{l}{Project age} & 0.00 & 365.03 & 884.32 & 1593.42 & 5487.76 & 1103.76\\
    \multicolumn{2}{l}{} &\multicolumn{2}{l}{Number of contributors} & 1.00 & 2.00 & 4.00 & 9.00 & 345.00 & 9.70\\
    \multicolumn{2}{l}{Deprecated Packages (844)} &\multicolumn{2}{l}{Number of releases} & 2.00 & 4.00 & 8.00 & 15.00 & 324.00 & 13.86\\
    \multicolumn{2}{l}{} &\multicolumn{2}{l}{Duration since last commit} & 375.34 & 665.37 & 1080.07 & 1680.45 & 4191.07 & 1271.04\\
    \multicolumn{2}{l}{} &\multicolumn{2}{l}{Delta of downstream dependencies} & -87.00 & 0.00 & 0.00 & 0.00 & 14.00 & -0.96\\
    \multicolumn{2}{l}{} &\multicolumn{2}{l}{Number of unresolved issues} & 0.00 & 0.00 & 0.00 & 0.00 & 88.00 & 0.95\\
    \midrule
    \multicolumn{2}{l}{} &\multicolumn{2}{l}{Project stars} & 0.00 & 1.00 & 3.00 & 16.00 & 7567.00 & 61.78\\
    \multicolumn{2}{l}{} &\multicolumn{2}{l}{Project age} & 0.00 & 58.15 & 318.35 & 948.28 & 12975.92 & 663.14\\
    \multicolumn{2}{l}{} &\multicolumn{2}{l}{Number of contributors} & 1.00 & 1.00 & 2.00 & 5.00 & 284.00 & 6.15\\
    \multicolumn{2}{l}{Brothers of Deprecated Packages (679)} &\multicolumn{2}{l}{Number of releases} & 2.00 & 3.00 & 5.00 & 11.00 & 1005.00 & 11.30\\
    \multicolumn{2}{l}{} &\multicolumn{2}{l}{Duration since last commit} & 372.72 & 666.66 & 1028.16 & 1607.91 & 4185.62 & 1253.32\\
    \multicolumn{2}{l}{} &\multicolumn{2}{l}{Delta of downstream dependencies} & -6.00 & 0.00 & 0.00 & 0.00 & 46.00 & 0.09\\
    \multicolumn{2}{l}{} &\multicolumn{2}{l}{Number of unresolved issues} & 0.00 & 0.00 & 0.00 & 0.00 & 53.00 & 0.83\\
    \bottomrule
    \zq{maybe explain the table}
    % Note: *$p<0.05$; **$p<0.01$; ***$p<0.001$
  \end{tabular}
\end{table*}

\noindent\subsection{Package-Level Deprecation Patterns (RQ1)}
\noindent\textbf{Dataset Overview.}
We constructed our inactive dataset by selecting 89,193 packages from the total of 415,151 packages on PyPI, along with their corresponding GitHub repository data, as listed in table~\ref{tab:definitions}.
% From the total 415,151 packages on PyPI, we finally form our inactive dataset with 89,193 inactive packages and their corresponding GitHub repository data as listed in table~\ref{tab:definitions}. 
Among the 89,193 inactive packages, 52,250 (58.6\%) packages contain vulnerabilities either in themselves or in direct and transitive dependencies. 
For the 27,795 (31.2\%) packages without vulnerabilities, we found that they have no upstream dependencies in the dependency network. 
These results highlight the prevalence of vulnerabilities in the Python ecosystem.
It is worth noting that we provide this dataset for further research on package-level deprecation and OSS sustainability.
Here we show more statistics of the dataset in Table~\ref{tab:Overview}. 

To have intuitive cognition of our dataset, let's see Table~\ref{tab:Overview}.
In Table~\ref{tab:Overview}, we record the distribution of the characteristics in the entire dataset, the deprecated packages in the dataset and the brothers of deprecated packages that we selected in section~\ref{sec:estimation}.\zq{explain the 25\% 50\% 75\%}
In terms of project stars, project age, number of contributors and number of releases, these metrics can be indicators of maintenance level before being inactive.
We observe that deprecated packages have a better score in terms of these metrics compared to the other two groups, which indicates that deprecated packages may have a better maintenance level before being inactive.
% \zq{need more discussion}

% \zq{x=[total, unlabeled, deprecated, not deprecated], y=[age, last commit to now, contributor, release amount, stars]}

\noindent\textbf{Deprecation Pattern.} In our inactive dataset, we search for a keyword list in README and issues since the last commit, and there are 1,921 repositories that contain the keyword we searched. 
We manually inspected the 1,921 repositories and eventually found deprecation announcements in 844 (44\%) repositories, which is only 9.5\textperthousand \ of the entire inactive dataset. \zq{a Donut pie chart here}

% In metrics of project stars, project age, number of contributors and number of releases, deprecated packages have a better score compared to the other two groups.
% These metrics indicate maintenance level before being inactive.
% We have 
% we curve the percentage of some star values for the complete dataset and the data points with deprecation announcements that we labeled.
% In the all-data points group, Projects with more than 7 stars do not surpass those with less than 7 stars.
% While in the deprecation group, projects with more than 7 stars stand as the majority of the group, for up to 60\% of the group. \zq{need to be refined}

% \begin{figure}[ht]
% 		\centering
% 		\includegraphics[width=0.90\linewidth]{Figures/deprecation+characteristics.pdf}
% 		\caption{Basic characteristics of the dataset. \zq{need to be refined}}
% 		\label{fig:basic_characteristics}
% \end{figure}

Among those 844 packages with deprecation announcements, 739 announcements were made in README, 127 of them were made in GitHub issues, and 22 of them contain the announcement both in README and GitHub issues.

\begin{figure*}
    \centering
    % \includegraphics{}
    \label{fig:rationales}
    \begin{tikzpicture}

    \pie[
        color = {
            yellow!90!black, 
            green!60!black, 
            blue!60, 
            red!70,
            gray!70,
            teal!20},
        text = legend
    ]
    {
        2.1/Legal problem,
        22.7/Broken dependencies,
        7.8/Presence of bugs or vulnerabilities,
        45.4/There are better alternatives,
        17.7/No time and interest,
        4.3/Lack of resource}
    \end{tikzpicture}
    \caption{Rationales for Deprecation}
\end{figure*}

We further categorized the rationales provided in 141 deprecation announcements.
As Figure~\ref{fig:rationales} shows, the most frequent rationale for deprecations is the existence of better alternatives, which was reported in 64 (45.4\%) deprecation announcements.
% 64 (45.4\%) of the packages were deprecated since there were already better alternatives that are better in the aspect of popularity or functionality.
Then, 32 (22.7\%) of the packages were deprecated due to breaking dependencies, e.g., the dependencies do not work as before, and the user policy has changed, which is the second most frequent rationale.
Noted that the dependencies here refer to not only packages on PyPI but also include third-party APIs, software components and data sources that the packages subscribe to.
25 (17.7\%) of the packages were deprecated since the maintainers have no time and interest anymore.
In addition,
11 (7.8\%) of the packages were deprecated due to vulnerabilities or bugs in the code.
6 (4.3\%) of the packages reported deprecation for lack of resources to provide further support.
% 3 (2.1\%) of the packages were deprecated for bugs that can not be fixed, further xx of the packages were deprecated since they contain vulnerabilities.
3 (2.1\%) of the packages were deprecated due to legal problems, e.g., experiencing a police raid and limitation of the contract. 
% \zq{list rationales here}
% 2 (1.4\%) of the packages were deprecated since they have been renamed and will contribute to the new package instead of the old one.

\begin{table*}
  \centering
  \caption{Summaries of linear mixed-effect model regressions
  % estimating the effect of having a deprecation and its characteristics on minimizing delta of downstream and new unresolved issues. We report the coefficient estimates and their standard errors in parentheses. \zq{layout needs to be improved}
  }
  \label{tab:results}
  \begin{tabular}{llllll}
    \toprule
    \multicolumn{2}{l}{} &\multicolumn{2}{c}{delta of downstream} &\multicolumn{2}{c}{number of unresolved issues (log)}\\
    \cmidrule(lr){3-4}\cmidrule(lr){5-6}
    \multicolumn{2}{l}{} & Model I & Model II & Model III & Model IV \\
    \cmidrule(lr){3-6}
    % \multicolumn{2}{l}{\textbf{Outcome Variables}}& & & & & & \\
    % \texttt{{\char'134}table*}& 400& For wider tables & &  & &\\
    \multicolumn{2}{l}{\textbf{Repository Characteristics}}& & & & \\
    \multicolumn{2}{l}{Project stars (log)} & \ 0.01 & \ 0.02&  \ 0.16 *** & \ 0.15 ***\\
    \multicolumn{2}{l}{Project ages (log)} & \ 0.01 & \ 0.02&  -0.03 *** & -0.03 **\\
    \multicolumn{2}{l}{Number of contributors (log)} & -0.58 ***& -0.62 ***&  \ 0.08 *** & \ 0.07 *** \\
    \multicolumn{2}{l}{Number of releases (log)} & -0.19 & -0.20& -0.02 & -0.02 \\
    \multicolumn{2}{l}{Duration since last commit (log)} & \ 0.11 & \ 0.04 & \ 0.08 *** & \ 0.05 *\\
    \multicolumn{2}{l}{\textbf{Deprecation Characteristics}}& & & &  \\
    \multicolumn{2}{l}{Has deprecation}  & -0.81 *** & & -0.15 *** &\\
    \multicolumn{2}{l}{Has replacement} &  & \ 0.54 & & -0.06    \\
    \multicolumn{2}{l}{Has rationale} &  & -1.24 **& & -0.06 \\
    \multicolumn{2}{l}{Published in README} &  & -1.02 ***&  & -0.16 *** \\
    \multicolumn{2}{l}{Published in Issues} &  & -0.13 &  & \ 0.24 ***  \\
    % \midrule
    % \multicolumn{2}{l}{Num. obs.} & 1,523 & 1,523 & 1,523 & 1,523 \\
    % \multicolumn{2}{l}{$R^2_m (R^2_c)$} & 1,523 & 1,523 & 1,523 & 1,523 \\
    \bottomrule
    Note: *$p<0.05$; **$p<0.01$; ***$p<0.001$
  \end{tabular}
\end{table*}


% \begin{figure*}[ht]
% 		\centering
% 		\includegraphics[width=0.90\linewidth]{Figures/delta_issues.pdf}
% 		\caption{delta of downstream and unresolved issues. \zq{need to be refined}}
% 		\label{fig:delta_issues}
% \end{figure*}


\noindent\subsection{Deprecation Effects on Unresolved Issues and Dependents (RQ2) \zq{conclusion is needed}}
Our initial investigation in Table~\ref{tab:Overview} revealed that the number of dependents for projects with deprecation announcements decreased compared to those without such announcements. 
\zq{need to be refined.} 

To further confirm the results, we build lmer models to see how having a deprecation announcement can affect the gain of the delta of downstream dependencies and unresolved issues.
Here we see the summary in Table~\ref{tab:results}.

In Table~\ref{tab:results}, we record the estimated coefficient of the predictors in four models.
Let's start with Model I, the results show that having a deprecation announcement shows statistically significant negative effects of delta of downstream dependencies gain.
On average, having a deprecation announcement corresponds to approximately 0.81 downstream package decreases.
The value is no more than one may due to 595 (70\%) of the deprecated packages that have had no downstream dependencies on PyPI ever since the first release.
However, there may be a lot of downstream projects that are not in PyPI, which are not in our observation.
To interpret the effect of the number of unresolved issues, we turn to Model III.
Similarly, the deprecation announcement also shows statistically significant negative effects of unresolved issues gained. 
On average, a deprecation announcement corresponds to approximately a 7\% decrease in unresolved issues.
Note that the coefficient should be interpreted as the percentage of increase or decrease since the number of unresolved issues is log-scaled.
Overall, having a deprecation announcement exhibited a strong negative coefficient with the gain of the downstream dependencies and unresolved issues, thus further confirming the effect and necessity. \zq{more detail}

% \begin{figure}[ht]
% 		\centering
% 		\includegraphics[width=0.90\linewidth]{Figures/deprecation+characteristics.pdf}
% 		\caption{replacement and rationales. \zq{need to be refined}}
% 		\label{fig:basic_characteristics_RQ3}
% \end{figure}

\noindent\subsection{Characteristics of Effective Deprecation Announcements (RQ3)}
We extend the original lmer model to further inspect the effect on different characteristics of the deprecation. 
The estimated coefficient is recorded in Model II and Model IV in Table~\ref{tab:results}

Let's start with discussing the publishing manner of deprecation announcements, which is in README or in Issues.
Which current publishing manners make a good and effective deprecation?
In Model II, the results show statistically significant negative effects of publishing in README.
That is, a deprecation announcement published in 
README corresponds to approximately 1.02 downstream package decreases on average.
The effect of having a deprecation published in GitHub issues is unclear since the model does not show statistical significance on the predictor.
In terms of the number of unresolved issues, we turn to interpret the results of Model IV.
Similar to that in the delta of downstream dependencies, a deprecation announcement published in README has a statistically negative impact on the unresolved issues gained.
On average, a deprecation announcement published in README corresponds to a 16\% decrease in the number of unresolved issues.
While a deprecation announcement published in GitHub issues can not stop the number of unresolved issues gained with statistical evidence.
Overall, the results show that the publishing manner is essential.
Deprecation announcements released in README can significantly stop consumers and potential consumers from adopting the deprecated packages, thus further preventing issues with no reply.
While the announcements released in GitHub issues can not stop the situation.

Now we discuss what contents in the deprecation announcement make a effective deprecation announcement.
Specifically, we discuss the effect of having a replacement and having a rationale in the deprecation announcement.
We look at Model II, the estimated coefficients show statistically significant negative effects of a deprecation that contains a rationale, which corresponds to 1.24 downstream packages decrease.
While the effect of having a replacement is not clear.
Next, we turn to Model IV, we note that both deprecation announcements that have a replacement and have a rationale do not show statical significance in reducing the number of unresolved issues. \zq{any explanation?}

% From the result of model II, it is suggested that the deprecation declared in README reduces the negative effect more than that in GitHub issues, which validates the hypothesis of having a conspicuous deprecation announcement can have a significant effect on preventing adoption.
% And the result of Model IV shows that it can further prevent consumers from the situation where they seek help but receive no reply.

% while there are too few samples of having a rationale, and is highly correlated with the characteristics of having a replacement, thus we can not estimate the effect of having a rationale.
% It is easy to verify that the deprecation announcement can significantly reduce the downstream adoption and unresolved issues.





==> 07Disscussion.tex <==
\section{Discussion and Implications}
In this section, we summarize the main results of the paper and give an in-depth discussion of their implications.

\noindent\textbf{More than half of inactive packages in the Python ecosystem contain vulnerabilities.} 
As our result shows \zq{which results}, 52,250 (58.6\%) inactive packages in the Python ecosystem contain vulnerabilities. 
Of those packages that adopted third-party dependencies, only 9,148 (15\%) are not involved in vulnerabilities.
Though 2,857 (95.3\%) of the open source vulnerabilities in PyPI were fixed in a later version, 
% \zq{add to methods}
the old and vulnerable versions can still affect the downstream packages if downstream does not update their requirements and specify the new version of dependencies.
This implies that many affected projects may be unaware of the vulnerability to their software, as well as the corresponding patch \cite{kula2018developers}.
The situation can easily happen on inactive packages since they are continually under low maintenance and thus have no ability to keep the dependencies up-to-date.

\noindent\textbf{Only 9.5\textperthousand \ of inactive projects seldom make deprecation declarations.}
% As Coelho et al. interviewed some of the members of popular GitHub projects that are no longer maintained or without any commit for the last year \cite{coelho2017modern}. 
% The results show that 86\% of the developers confirm the abandonment of the projects.
Though a large proportion of packages in the Python ecosystem are in the inactive state, there is only 9.5\textperthousand \ of them make a deprecation declaration, which may easily expose their consumers or potential consumer to risks (e.g., encounter bugs or vulnerabilities without support from the developer). 
Although there are completed projects in the inactive projects, however, there were rare cases and most of the inactive projects were confirmed as abandoned as reported by Coelho et al. \cite{coelho2017modern}.
In summary, there is a large proportion of inactive and probably abandoned projects in the Python ecosystem without an explicit deprecation declaration to discourage consumers and potential consumers from adopting the package.

\noindent\textbf{Projects with more contributors before being inactive are more likely to make a deprecation declaration.} 
We observed that the inactive projects with more contributors are more likely to have a deprecation declaration.
As OSS has a life cycle from inception to deprecation \cite{valiev2018ecosystem}. 
Most of the projects do not have a good and complete end in their late stage in the life cycle, which are reaching the deprecation messages to the consumers and help them find out the alternatives since the key contributors have been disengaged \zq{TFDD}.
% Thus, to help an open-source project have a complete life cycle, it heavily relies on maintenance resources (e.g., number of contributors). \zq{reference on life cycle}
The situation shows the urgent need for automated tools to help the project without enough resource to finish the life cycle, especially when the key contributors have been disengated, automatically evaluate the severity and then decide whether deprecate the project, and if so, then help downstream find out the replacement.
This can significantly decrease the consumers' confusion on whether to adopt the package or not. \zq{need to be refined}

\noindent\textbf{Less than half of the deprecated package provides alternatives, and rationales are even less.}
In the results of \textbf{RQ1}, only 406 (48.1\%) of the deprecation declarations provide an alternative, and 141 (16.7\%) provide a rationale for the deprecation.
While the package-level and release-level deprecation mechanism of .NET forces the developer to provide a reason for the deprecation, it is optional to provide a replacement in the current Python ecosystem.
As no existing package-level deprecation mechanism for the Python ecosystem, whether a replacement and rationale are provided mostly depends on the consciousness of the developers.
Less information for the consumers after encountering a deprecation of dependencies, which increases the decision cost, i.e., to perform migration or keep the code remains.
We acknowledge that it could be difficult for both developers and consumers to find out an alternative, therefore, an automated tool might be needed.

% \noindent\textbf{More details about replacement (not all replacements are in PyPI, which indicates that the migration recommendation should include a larger scale).}
% From the replacements given in the deprecation announcements, it is not always that the replacements come from the PyPI ecosystem (i.e., other PyPI packages).
% There is a non-negligible ratio of the replacements that come from other GitHub repositories that do not originate from PyPI.
% Our results also discovered the possibility that the replacements come from a third-party service (e.g., API from other service provider except for GitHub and PyPI).
% The various sources of replacements come up with new challenges for the Migration recommendation and automated Migration. \zq{maybe more details}

\noindent\textbf{Presence of better alternatives is the most frequent rationale for the deprecation. In addition, legal problems and broken dependencies need attention from OSS community and academia.} \zq{need to be refined}
The rationales of the deprecation are also interesting.
Despite the most common reason which is "no time and interest", the study results also show other possibilities different from prior works.
We can see a non-negligible ratio of rationales claiming that the breaking upstream led to the deprecation.
The upstream here is not necessarily be the PyPI package that explicit define in the requirements.
It could be the data source, the API, or the component from other software.
These upstreams can break due to many reasons, for example, the upstream does not work as before, or the user policy is changed. 
In these situations, we call for researchers to focus on not only breaking changes within the ecosystem but also outside the ecosystem in the future.
We also notice that there are projects that explain their deprecation for accident factors (e.g., police raids, lack of resources that support the projects). 
This indicates that risk management and legal issues are quite a plain area in OSS research, which might help promote the sustainability of the OSS community.

\noindent\textbf{Deprecation declaration can significantly reduce the negative impact of lacking maintenance.}
From the results in \textbf{RQ2}, we show how having a deprecation declaration reduces the negative impact of lacking maintenance.
First, we discuss the delta of downstream dependencies.
As we show that more than half packages in our inactive package dataset contain vulnerabilities, and it is unlikely to re-active the package and update the dependencies.
Discouraging downstream dependencies by adopting inactive packages to stop vulnerability propagation is essential.
In this aspect, projects with depreciation declarations can significantly reduce downstream dependencies, which stop propagation well.
Then, we turn to discuss the effect of reducing unanswered issues.
The results also show that having a deprecation declaration can significantly reduce unanswered issues.
% xxx

\noindent\textbf{Providing a rationale makes an effective deprecation declaration.}
% The results seem counterintuitive.
We investigate the factors that contribute to the gain of downstream dependencies and unresolved issues in \textbf{RQ3}.
The results show that the deprecation declarations that provide a rationale for the deprecation can ease the gain with statistical significance, which indicates that providing a rationale in the deprecation mechanism makes an effective deprecation declaration.
Here we give a possible explanation.
For consumers who have already adopted the deprecated package in their projects, it is hard to decide whether refactor the projects and migrate to the alternative since it could induce costs.
When a deprecation declaration provides a rationale, it is more persuasive in discouraging consumers from using the package.
% When consumers consider whether to adopt or migrate to the alternative, 
% When a deprecation announcement with a rationale could be more persuasive to consumers.
Thus easing the gain of downstream dependencies and unresolved issues.
Among the current implementations of package-level and release-level deprecation mechanisms from four popular ecosystems, namely Crates.io for Rust, Nuget for .NET, Packagist for PHP and npm for JavaScript, only the deprecation mechanism of Nuget requires rationales when performing deprecation \cite{cogo2021deprecation}.
The situation indicates the necessity of requiring a rationale in the depreciation mechanism is not a consensus yet.
This finding strengthens the necessity of requiring rationales in the package-level deprecation mechanism, which can serve as a guideline for the implementation of the package-level deprecation mechanism for the Python ecosystem.
% Performing migration and refactoring induces huge costs to consumers.
% If there is more information about why the developers of the deprecated package discourage consumers to use the packages, consumers may be more willing to pay the costs.

\noindent\textbf{Making it as conspicuous as possible.}
As we can see in the results of estimating the publishing channels, having an declaration in README can perform better than that in issues to reduce the negative impact of no more maintenance.
Though the conclusion is quite intuitive, we can still highlight that when developing a package-level deprecation mechanism in the future.
As we mentioned in \zq{?}
In addition, it is also promising to develop an automated tool to mine the deprecation message including but not limited to GitHub issues, and display it in more conspicuous places.
% \zq{more?}

\noindent\textbf{Insuficiency of the current propagation model.}
Though there is a deprecation declaration in the corresponding GitHub repository, some of the projects that experiencing an increase in downstream dependencies imply the insufficiency of the current deprecation pattern.
Compared to the deprecation mechanism in other ecosystems (e.g., npm for JavaScript) that collect deprecation messages and push them to every consumer that wants to install the packages in a unified manner, the current deprecation pattern in the Python ecosystem makes high demands on consumers in proactivity.
There is no unified paradigm to release a deprecation declaration, especially in the aspect of the position.
Since not everyone finds the corresponding home page and reads the document and reads every single issue, especially when there is no sign that the package he is going to adopt is no longer being maintained anymore.
Even the deprecation mechanism of npm is not efficient enough, since it can only prevent consumers that did not adopt the package before from adopting the deprecated packages. \zq{a reference here}
It does not have efficient methods to send a warning to those who have already adopted the package and will not need to experience an installation after the package was deprecated, where the deprecation mechanism mostly works.
The challenge remains open for the design of the Python deprecation mechanism.

% \zq{more implications?}
